Multiphase-Diff: Diffusion-Based Generative Modeling for High-Contrast Multiphase Physical Systems with Sharp Interfaces

Physics-constrained diffusion for high-contrast, sharp-interface multiphase fields faces three coupled difficulties. At coefficient jumps, expanded pointwise strong-form PDE residuals contain singular gradient terms that can penalize physical interfaces. Under extreme contrast, low-magnitude phases may fall below the diffusion noise floor and be erased, misscaled, or generated with negative coefficients, while a global likelihood scale allows high-magnitude phases to dominate supervision. We therefore propose Multiphase-Diff, which makes three corresponding contributions: (i) a conservative flux residual that avoids differentiating discontinuous coefficients and enforces discrete conservation; (ii) an analytic bijective representation that maps low-amplitude signals to order-one latent scales and guarantees coefficient positivity through exponential decoding; and (iii) a Jacobi-preconditioned likelihood that normalizes local residual scales for balanced supervision. Experiments on three complementary multiphase benchmarks demonstrate the superiority of Multiphase-Diff over seven baselines in both physical and distributional fidelity and its robustness across phase contrasts and compositions, establishing its effectiveness for scientific sample generation in this challenging regime.

==> paper_intro_to_method.tex <==
\title{Multiphase-Diff: Physics-Informed Generative Diffusion for Multiphase Physical Systems}


\section{Introduction}
\label{sec:introduction}

Learning generative models that capture the structure of complex scientific
data while respecting known physical principles is a central objective of AI
for science~\cite{karniadakis2021physics}. In scientific domains, fidelity is not
exhausted by statistical agreement with observed data: generated states must
also remain within the physically admissible space defined by conservation
laws, constitutive relations, and boundary and interface conditions. This
requirement becomes particularly demanding in multiphase systems, where
extreme material contrasts and sharp interfaces couple heterogeneous
statistics with nonsmooth physics.

Denoising diffusion probabilistic models~\cite{ho2020ddpm,sohldickstein2015nonequilibrium} have become the dominant approach to generative
modeling because they are stable to train, cover modes well, and produce
high-fidelity samples~\cite{nichol2021improved,song2021scorebased}. They
are, however, purely data-driven: the denoising objective only teaches the
model to reproduce the statistical patterns of the training data. A diffusion
model therefore attains distributional fidelity, in that its samples look
like the data, but it carries no guarantee of physical fidelity. A generated
field may look plausible while violating conservation of mass or charge, and
such a field cannot be used as a physical state in a scientific pipeline.

To bridge this gap, recent studies incorporate governing partial differential
equations (PDEs) into diffusion models so that generated fields more closely
satisfy physical constraints. For example, residuals derived from the Darcy
or Navier Stokes equations can guide the generation of fluid fields toward
physically admissible states. Existing approaches enforce such constraints
at different stages. Physics guided diffusion uses the residual as
conditioning information~\cite{shu2023physics}, CoCoGen corrects
samples during inference~\cite{jacobsen2025cocogen}, and PIDM
incorporates a residual likelihood during
training~\cite{bastek2025pidm}. These methods have been evaluated primarily on smooth fields or
systems with moderate heterogeneity. More recent work has begun to consider less regular physical fields.
DiffusionPDE~\cite{huang2024diffusionpde} jointly models coefficient and solution
fields and considers a binary Darcy coefficient. Its main focus, however, is
forward and inverse recovery from sparse observations, with physics imposed
through guidance during inference and under moderate coefficient contrast.
FunDiff~\cite{wang2026fundiff} develops generative modeling in function spaces
and considers Burgers solutions with steep fronts as well as linear
elasticity fields with material interfaces. It does not address the joint
generation of an extremely high contrast discontinuous leading coefficient
and its corresponding solution. Although these studies advance physical
generative modeling in important directions, none is designed specifically
for the simultaneous challenges of high material contrast, sharp interfaces,
and physical consistency between coefficient and solution fields. This
demanding and practically important regime is the focus of our work.

High-contrast, sharp-interface multiphase fields are difficult for
diffusion-based physics-informed generation in three specific and distinct
ways.

\noindent\textbf{Interface irregularity.} Conventional pointwise strong-form residuals
implicitly assume sufficient coefficient smoothness. At sharp material
interfaces, coefficient jumps invalidate this assumption and can create
artificial interface penalties, causing physics supervision to blur or
suppress the discontinuities it should preserve.

\noindent\textbf{Low-amplitude phase under-resolution.} In a high-contrast field, the
low-magnitude phase can be much weaker than both the diffusion noise and the
model's denoising error. Absolute-error training also underweights its
relative accuracy, so the phase may be erased, shifted to the wrong
magnitude, or pushed into physically inadmissible negative values.

\noindent\textbf{Residual-scale heterogeneity.} Physical residuals can vary by orders of
magnitude across phases and samples because their local coefficient and flux
scales differ. A single global likelihood scale is therefore dominated by
high-flux regions and cannot provide balanced physics supervision throughout
the field.

To solve these three problems for the generation of high-contrast
sharp-interface multiphase fields, we propose \textbf{Multiphase-Diff}, whose
contributions are as follows.

\begin{enumerate}
\item We introduce a \textbf{conservative flux residual} that removes the interface
   irregularity of the pointwise strong form. Written as a finite-volume
   two-point flux with a harmonic face coefficient, the residual never
   differentiates the coefficient field, is well posed at coefficient jumps
   of arbitrary contrast, and is discretely conservative.
\item We develop an \textbf{analytic bijective representation} (a logarithmic map for
   the coefficient and an inverse-hyperbolic-sine map for the solution) that
   lifts the low-amplitude phase above the diffusion noise floor and
   guarantees positivity by construction, and we pair it with a
   \textbf{Jacobi-preconditioned residual likelihood} that normalizes the residual
   by the local flux capacity, so that a single scale supervises phases and
   samples whose residual magnitudes differ by orders of magnitude.
\item We validate Multiphase-Diff with extensive experiments on three
   complementary discontinuous multiphase benchmarks and against a broad set
   of baselines, and we demonstrate its superiority and effectiveness,
   including its robustness across phase contrast and phase composition.


\end{enumerate}

\section{Related Work}
\label{sec:related-work}

\subsection{Generative Modeling of Multiphase Physical Systems}

Generative models are increasingly used to represent the geometric and
statistical complexity of multiphase physical systems. In the subsurface,
latent diffusion models parameterize geological facies for history matching
and data assimilation~\cite{lee2025facies,difederico2025latent}. For
heterogeneous materials, generative adversarial networks reconstruct
three-dimensional multiphase electrode microstructures~\cite{gayonlombardo2020pores}, while diffusion models reconstruct two- and three-dimensional random
media and condition their morphology on prescribed permeability ranges~\cite{lyu2024microstructure}. Recent diffusion models also generate pore-scale images that
contain both the solid geometry and multiple fluid phases~\cite{zhu2025porescale}, as well as two- and three-phase material microstructures
conditioned on volume fractions and tortuosities~\cite{baishnab2025multiphase}.
Related approaches use diffusion for property-aware microstructure design
~\cite{vlassis2023microstructures} and topology optimization~\cite{maze2023topology,giannone2023aligning}. Collectively, these studies demonstrate that modern
generative models can reproduce sharp phase morphology, connectivity,
spatial correlations, and selected effective properties.

Their treatment of physics, however, is generally centered on the generated
morphology. Physical information is supplied through an aggregate
conditioning variable or design objective, or is evaluated after generation
by a separate simulator. Even when the training samples originate from a
physics-based process, these approaches do not typically generate a local
state field together with its coefficient field and enforce that each
generated pair satisfies the governing conservation law during diffusion
training. Consequently, matching phase statistics or even the distribution
of an effective property does not by itself establish local coefficient--
solution consistency, particularly at sharp interfaces under extreme
contrast. Multiphase-Diff addresses this complementary gap. It jointly
generates the coefficient and solution fields, evaluates an
interface-consistent conservative flux residual after decoding them to
physical space, and balances the resulting heterogeneous residual scales
through local preconditioning. The goal is therefore not only morphological
fidelity, but joint distributional and physical fidelity for each generated
multiphase sample.

\subsection{Physics-Constrained Diffusion Models}

A growing line of work injects physical constraints into diffusion models,
and can be organized by where the constraint is applied. At training time,
PIDM adds a residual likelihood derived from the virtual-observable view of
constraints~\cite{bastek2025pidm,rixner2021virtual}.
As conditioning, physics-guided diffusion supplies the residual gradient as
an input signal~\cite{shu2023physics}, following the guidance
literature~\cite{dhariwal2021diffusion,ho2022classifierfree}. At inference
time, CoCoGen corrects the sample by residual
descent~\cite{jacobsen2025cocogen} and DiffusionPDE guides the noisy sample by backpropagating
the residual through the denoiser~\cite{huang2024diffusionpde}. In function space,
FunDiff places the physics in a physics-informed autoencoder and generates
with a latent diffusion model trained using rectified
flow~\cite{wang2026fundiff}. Further variants evaluate residuals in
a spectral basis~\cite{gallon2026spectral}, distill PDE satisfaction into few-step
generators~\cite{zhang2025distillation}, stabilize physics-informed
consistency models against degenerate solutions~\cite{chang2026stabilizing}, and
balance the physics and data objectives by Pareto analysis or conflict-free
gradients~\cite{baldan2025physics,tauberschmidt2025finetuning,liu2025config}. These methods have not been validated as a unified solution
for the joint generation of a discontinuous leading coefficient and its
solution under extreme phase contrast. The limitation is not that every
spectral method is mathematically incompatible with discontinuities: weak
spectral formulations, domain-decomposed schemes, and
discontinuity-adapted bases can all be constructed. Rather, truncated smooth
Fourier representations can suffer Gibbs oscillations at sharp jumps, while
existing physics-informed spectral diffusion has been demonstrated on
Poisson, Helmholtz, and incompressible Navier--Stokes settings rather than on
high-contrast discontinuous leading coefficients. Related operator-learning
work has therefore explored discontinuity-adapted representations such as
Walsh--Hadamard bases~\cite{cavallazzi2026walsh}, and
PINN studies have introduced region-aware treatments for discontinuous
permeability~\cite{aziz2025selfadaptive}. A second unresolved issue is that a globally
weighted residual does not adapt to the per-phase and per-sample scale
disparity induced by extreme contrast. Multiphase-Diff addresses these
specific gaps by placing an interface-consistent conservative residual,
made locally scale-balanced through preconditioning, inside the generative
objective.


\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Denoising Diffusion Probabilistic Models}

A denoising diffusion probabilistic model~\cite{ho2020ddpm} defines
a fixed forward process that gradually corrupts a clean sample $x_0$ into
noise, and learns a reverse process that removes the noise step by step.

\noindent\textbf{Forward process.} Given a variance schedule $\beta_1,\dots,\beta_T$, with
$\alpha_t=1-\beta_t$ and $\bar\alpha_t=\prod_{s=1}^{t}\alpha_s$, the forward
process adds Gaussian noise so that the noisy sample at step $t$ can be
written in closed form from the clean sample,

\begin{equation}
\begin{aligned}
q(x_t\mid x_0)
  &=\mathcal N\!\left(
      x_t;\sqrt{\bar\alpha_t}\,x_0,
      (1-\bar\alpha_t)I\right),\\
x_t
  &=\sqrt{\bar\alpha_t}\,x_0
    +\sqrt{1-\bar\alpha_t}\,\epsilon,
\qquad \epsilon\sim\mathcal N(0,I).
\end{aligned}
\tag{1}
\end{equation}

As $t$ increases, $\bar\alpha_t$ decreases from near one to near zero, so
$x_T$ is approximately standard Gaussian noise that retains no information
about $x_0$.

\noindent\textbf{Reverse process.} Generation runs the process backward. Starting from
$x_T\sim\mathcal N(0,I)$, the model denoises step by step using a learned
Gaussian transition
$p_\theta(x_{t-1}\mid x_t)=\mathcal N(x_{t-1};\ \mu_\theta(x_t,t),\ \Sigma_t I)$,
whose posterior mean, given an estimate $\hat x_0$ of the clean signal, is

\begin{equation}
\begin{aligned}
\mu_\theta(x_t,t)
  &=\frac{\sqrt{\bar\alpha_{t-1}}\,\beta_t}
          {1-\bar\alpha_t}\,\hat x_0\\
  &\quad+
    \frac{\sqrt{\alpha_t}(1-\bar\alpha_{t-1})}
         {1-\bar\alpha_t}\,x_t,\\
\Sigma_t
  &=\frac{1-\bar\alpha_{t-1}}
          {1-\bar\alpha_t}\,\beta_t.
\end{aligned}
\tag{2}
\end{equation}

Repeating this transition from $t=T$ down to $t=1$ turns Gaussian noise into a
sample from the learned data distribution. The network is trained so that its
reverse transitions match the forward posterior, which reduces to a simple
regression objective introduced in Section 4.4.

\subsection{Elliptic Conservation Laws}

The physical systems we consider are described by a partial differential
equation on a spatial domain $\Omega\subset\mathbb R^2$. We use the family of
second-order elliptic conservation laws

\begin{equation}
\nabla\cdot\big(a(\boldsymbol\xi)\,\nabla u(\boldsymbol\xi)\big)=f(\boldsymbol\xi),
\qquad \boldsymbol\xi\in\Omega, \tag{3}
\end{equation}

with prescribed boundary conditions, where $a>0$ is a spatially varying
material coefficient, $u$ is the solution field, and $f$ is a source term.
This single form instantiates Darcy flow in porous media (with $a$ the
permeability and $u$ the pressure), fully developed viscous flow (with $a$
the viscosity and $u$ the axial velocity), and steady conduction (with $a$
the conductivity and $u$ the potential). In a multiphase medium the
coefficient $a$ is piecewise near-constant, with one value per phase, and the
phases meet at sharp interfaces. Across such an interface the physical
solution satisfies continuity of the field and of the normal flux,

\begin{equation}
[\,u\,]=0,\qquad [\,a\,\partial_n u\,]=0, \tag{4}
\end{equation}

so that the normal gradient of $u$ is itself discontinuous, jumping by the
ratio of the two coefficients. A generated pair $(a,u)$ is physically
consistent when it satisfies (3) together with the interface conditions (4).


\section{Methodology}
\label{sec:methodology}

Multiphase-Diff generates the coefficient-solution
pair $(a,u)$ with a diffusion model, but it makes three changes to the
standard recipe, one for each of the three difficulties identified in
Section 1. Figure 1 shows the pipeline. The pair is first mapped by an
analytic bijection $g$ into a latent representation $z_0=g(a,u)$ in which each
phase has an $O(1)$ amplitude and positivity is automatic (component I,
Section 4.1). The diffusion forward process, the network, and the data loss
all operate on $z_0$. At every step the network produces an estimate
$\hat z_0$ of the clean latent, which is decoded back to physical fields
$(\hat a,\hat u)=g^{-1}(\hat z_0)$ on which the physics is evaluated. The
physics is a conservative flux residual that is well posed at sharp
interfaces (component II, Section 4.2), preconditioned so that its scale is
uniform across phases and samples (component III, Section 4.3). The two terms
are combined into a single training objective (Section 4.4). Inference is
unchanged from a standard diffusion model, namely ancestral sampling in the
latent space followed by one decoding step.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{fig_framework.png}
    \caption{The Multiphase-Diff training pipeline. The diffusion path (top)
    operates on the latent representation produced by the analytic bijection
    $g$ (component I). The network estimate is decoded and scored by a
    conservative flux residual (component II) and a Jacobi preconditioner
    (component III). The three components solve, respectively, low-amplitude
    phase under-resolution, interface irregularity, and residual-scale
    heterogeneity. Inference is standard diffusion sampling followed by one
    decoding step.}
    \label{fig:framework}
\end{figure*}

\subsection{Analytic Bijective Representation}
\label{sec:representation}

Consider diffusing the
coefficient in raw physical units or after a global normalization that makes
the high phase $a_H$ of order one. For contrast
$\gamma=a_H/a_L$, the low phase then has amplitude
$a_L=O(\gamma^{-1})$. From the forward process (1), its
amplitude-dependent signal at step $t$ is
$\sqrt{\bar\alpha_t}\,a_L$, while the injected noise has standard deviation
$\sqrt{1-\bar\alpha_t}$. Consequently, its phase-conditioned signal-to-noise
ratio

\begin{equation}
\operatorname{SNR}_{L}(t)
=\frac{\bar\alpha_t\,a_L^2}{1-\bar\alpha_t}
\end{equation}

falls below that of the high phase by a factor $\gamma^2$ and can be
negligible for much of the trajectory. The MSE imbalance must be stated in
relative rather than absolute terms. If both phases have the same relative
reconstruction error $\rho$, their squared-error contributions are
$(\rho a_H)^2$ and $(\rho a_L)^2$, so the low phase contributes
$\gamma^{-2}$ as much loss. A conventional absolute representation
therefore devotes much less gradient pressure to multiplicative accuracy in
the low phase. Lacking a positivity constraint, an absolute denoising error
can additionally move a small positive value below zero.

We remove this problem by diffusing in an analytic
bijective latent space rather than in raw physical units. We apply
channel-wise invertible maps matched to the structure of each field,

\begin{equation}
\begin{aligned}
z_a&=\frac{\ln a-m_a}{s_a},\\
z_u&=\frac{\operatorname{asinh}(u/u_0)-m_u}
           {s_u^{\mathrm{tr}}}.
\end{aligned}
\tag{5}
\end{equation}

with an affine identity used for any channel that is already of order one.
The constants
$(m_a,s_a,u_0,m_u,s_u^{\mathrm{tr}})$ are fixed once from the training split.
The logarithm turns the multiplicative gap $\gamma$ between phases into an
additive gap $\ln\gamma$. More importantly, a small relative perturbation
$\delta a/a$ becomes, to first order, an additive perturbation
$\delta(\ln a)$, so comparable relative errors in different phases receive
comparable treatment in the latent loss. The inverse-hyperbolic-sine map
provides an analogous non-compressive representation for a signed solution,
behaving logarithmically at large magnitude and linearly near zero. Both maps
are lossless, non-learned, and exactly invertible, in contrast to a learned
latent space~\cite{rombach2022latent}, and a pointwise monotone transform
preserves the locations of spatial discontinuities. Decoding the coefficient
by $a=\exp(m_a+s_a z_a)$ guarantees $a>0$ by construction, so no generated
coefficient is inadmissible. Because the physics must be evaluated on
physical quantities, the residual of the following sections is always
applied to the decoded fields $g^{-1}(\hat z_0)$, not to the latent
variables.

\subsection{Conservative Flux Residual}
\label{sec:flux-residual}

Write the elliptic operator in
expanded strong form,

\begin{equation}
\nabla\cdot(a\nabla u)=a\,\Delta u+\nabla a\cdot\nabla u. \tag{6}
\end{equation}

In a multiphase medium $a$ is piecewise constant, so across an interface its
gradient $\nabla a$ is a singular distribution supported on the interface, not
an ordinary function, and the term $\nabla a\cdot\nabla u$ is undefined there
in the classical sense. Any pointwise finite-difference discretization of
$\nabla a$ on an interface cell returns a value of order $\Delta a/H$, where
$\Delta a$ is the coefficient jump, which scales with the contrast $\gamma$
and the grid resolution. This is a large artificial residual localized on the
interface cells. When such a residual is used as a training signal, it does
not measure a real physical violation; it penalizes the interface itself, and
the model responds by blurring the interface or lowering the high phase to
make the artifact smaller.

We instead measure the conservation law in flux form, which
never differentiates the coefficient. On the cell-centered grid we use a
two-point flux approximation with a harmonic average of the coefficient on
each face, the standard finite-volume scheme for strongly discontinuous
coefficients~\cite{aavatsmark2002multipoint,edwards1998finite},

\begin{equation}
\begin{aligned}
R_i(a,u)
  =\frac{1}{H^{2}}\Bigg(
    &\sum_{j\in\mathcal N(i)}
       T_{ij}(u_j-u_i)\\
    &+\sum_b T_{ib}(u_b-u_i)
    \Bigg)-f_i .
\end{aligned}
\tag{7}
\end{equation}

\begin{equation}
\begin{aligned}
T_{ij}&=\frac{2a_i a_j}{a_i+a_j},&
T_{ib}&=2a_i .
\end{aligned}
\tag{8}
\end{equation}

where $\mathcal N(i)$ are the neighbors of cell $i$ and the second sum runs
over boundary faces. Three properties make this residual suited to sharp
interfaces. First, it is well posed at any coefficient jump: the coefficient
enters only through the harmonic face mean $T_{ij}$, which is finite and
smooth in $(a_i,a_j)$ for all positive values and correctly limits the face
flux by the smaller of the two coefficients, so an arbitrary contrast
produces no spurious residual. Second, it is discretely conservative: the
flux across each internal face enters the balances of its two cells with
opposite signs, so it cancels in pairs, and the interface conditions (4) are
built into the scheme rather than being penalized. Third, it is consistent
with the data-generating discretization: the training fields are produced by
the same discrete operator, so their residual reaches the solver and storage
tolerance of the reference data rather than incurring a discretization
mismatch. The harmonic mean is defined only for positive coefficients, which
is exactly what the representation of Section 4.1 guarantees, so the two
components are not independent conveniences but are required together.

\subsection{Jacobi-Preconditioned Likelihood}
\label{sec:preconditioned-likelihood}

The residual (7) has the
physical units of the source $f$, and its characteristic local scale is set
by the flux capacity. Collecting the transmissibilities incident on cell
$i$ into the diagonal of the discrete operator,
$D_i=\sum_{j}T_{ij}+\sum_{b}T_{ib}$, which scales with the local coefficient,
a characteristic residual scale is
$D_i\,s_{\hat u}/H^2$, where $s_{\hat u}$ is a robust scale of the decoded
solution in the current sample. Between a high phase and a low phase,
$D_i$ can differ by orders of magnitude. Consequently, comparable relative
solution errors can produce absolute residuals on very different scales,
although the precise ratio also depends on local gradients and the source.
An unweighted residual likelihood $\|R\|^2$ is therefore biased toward
high-flux regions and high-amplitude samples, and a single scalar weight
cannot generally provide comparable supervision across all phases and
samples.

We remove this heterogeneity by dividing the residual
by the local flux capacity, which is a Jacobi (diagonal) preconditioning of
the discrete operator applied to the loss,

\begin{equation}
\begin{aligned}
S_i&=\operatorname{stopgrad}\!\left(
       \frac{D_i s_{\hat u}}{H^2}
       +\lVert f\rVert_\infty+\varepsilon
     \right),\\
\tilde R_i&=\frac{R_i}{S_i}.
\end{aligned}
\tag{9}
\end{equation}

where $s_{\hat u}$ is a per-sample robust scale of the decoded solution and
$\varepsilon$ is a small numerical floor. The entire denominator, including
$D_i$ and $s_{\hat u}$, is detached from the computational graph. Apart from
the fixed numerical floor, $\tilde R$ is dimensionless and invariant under
the joint rescaling $(a,u,f)\mapsto(\lambda a,u,\lambda f)$ admitted by the
equation. The normalization does not force every cellwise residual to be
exactly order one; rather, it expresses the violation relative to a
characteristic local operator and source scale. This substantially reduces
the phase- and sample-dependent dynamic range of the physics gradients and
allows one residual weight to be used across the evaluated cases. Detaching
the denominator prevents the model from reducing the normalized loss merely
by inflating the predicted coefficient or solution scale.

\subsection{Training Objective}
\label{sec:training-objective}

\noindent\textbf{From denoising to a constraint on the predicted clean field.} The original
diffusion objective trains the network to predict the noise $\epsilon$ that
was added at each step, minimizing
$\mathbb E\,\|\epsilon-\epsilon_\theta(z_t,t)\|^2$~\cite{ho2020ddpm}.
Because the forward relation (1) is affine, the noise, the noisy
sample, and the clean sample determine one another, and predicting the noise
is equivalent, up to a time-dependent factor, to predicting the clean latent
through

\begin{equation}
\hat z_0(z_t,t)
=\frac{1}{\sqrt{\bar\alpha_t}}
 \left[z_t-\sqrt{1-\bar\alpha_t}\,
 \epsilon_\theta(z_t,t)\right].
\tag{10}
\end{equation}

We therefore parameterize the network to output $\hat z_0(z_t,t)$ directly,
which is an estimate of the posterior mean $\mathbb E[z_0\mid z_t]$. The
denoising process can then be written as a time-weighted regression on the
predicted clean latent,

\begin{equation}
\mathcal L_{\mathrm{data}}
=\mathbb E_{t,z_0,\epsilon}\!\left[
 \lambda_t\,
 \lVert z_0-\hat z_0(z_t,t)\rVert^2
\right].
\tag{11}
\end{equation}

with the Min-SNR weighting $\lambda_t$~\cite{hang2023minsnr}. The key consequence
for us is that a clean-field estimate $\hat z_0$ is available at every
timestep, not only at the end of sampling. This is what lets us impose the
physics as a per-step constraint on the predicted clean field rather than on
an intermediate noisy state: at each step we decode $\hat z_0$ to physical
fields and evaluate the preconditioned residual there.

\noindent\textbf{Objective.} Following the virtual-observable view of constraints~\cite{rixner2021virtual,bastek2025pidm}, we treat the
physical constraint as a virtual observation $\hat r=0$ of the decoded clean
estimate. The exact posterior variance in (2) satisfies $\Sigma_1=0$, so it
cannot be used directly as a likelihood variance at the final diffusion
step. We therefore use the positive clipped variance
$\Sigma_t^{\mathrm{phys}}=\max(\Sigma_t,\Sigma_{\min})$, with
$\Sigma_{\min}>0$ fixed for all methods, and define

\begin{equation}
\begin{aligned}
q(\hat r=0\mid \hat z_0)
  =\mathcal N\!\Big(
    0;\;&\tilde R\big(g^{-1}(\hat z_0)\big),\\
        &(\Sigma_t^{\mathrm{phys}}/c)I
    \Big).
\end{aligned}
\tag{12}
\end{equation}

where $c$ is a single physics weight. The clipping preserves annealing over
the diffusion trajectory while keeping the final-step loss finite.
Maximizing this likelihood adds a preconditioned residual term to (11),
giving the Multiphase-Diff objective

\begin{equation}
\begin{aligned}
\mathcal L
=\mathbb E_{t,z_0,\epsilon}\Bigg[
  &\lambda_t
   \lVert z_0-\hat z_0(z_t,t)\rVert^2\\
  &+\frac{c}{2\Sigma_t^{\mathrm{phys}}}
   \left\lVert
   \tilde R\!\left(g^{-1}(\hat z_0(z_t,t))\right)
   \right\rVert^2
\Bigg].
\end{aligned}
\tag{13}
\end{equation}

Relative to a standard diffusion model, training adds only one decoding step
and one flux-residual evaluation per iteration, and sampling adds a single
decoding step. Because $g$ is a bijection, the representation itself loses no
information, and reference samples remain near-zero-residual feasible points
up to solver and storage tolerance. The added physics term nevertheless
generally changes the optimal finite-noise denoising estimator: even if every
clean sample satisfies the PDE, the conditional mean
$\mathbb E[z_0\mid z_t]$ need not remain on the nonlinear physical manifold.
The objective should therefore be interpreted as an explicit trade-off that
regularizes predicted clean fields toward physical consistency, not as a
term that is guaranteed to leave the data-only optimum unchanged.

\noindent\textbf{Training procedure.} Algorithm 1 summarizes one training step.

{\scriptsize
\begin{verbatim}
Algorithm 1  Multiphase-Diff training
Input: q(a,u), g, R, preconditioner,
       c, Sigma_min, {alpha_t}
1  repeat
2    (a,u) ~ q(a,u)
3    z0 = g(a,u)
4    t ~ Uniform{1,...,T}; eps ~ N(0,I)
5    zt = sqrt(abar_t) z0
        + sqrt(1-abar_t) eps
6    z0_hat = model(zt,t)
7    L_data = lambda_t ||z0-z0_hat||^2
8    (a_hat,u_hat) = inverse_g(z0_hat)
9    R_tilde = precondition(
         flux_residual(a_hat,u_hat))
10   Sigma_phys = max(Sigma_t,Sigma_min)
11   L = L_data
       + c ||R_tilde||^2/(2 Sigma_phys)
12   take gradient step on L
13 until converged
Sampling: DDPM in z-space;
          return inverse_g(z0).
\end{verbatim}
}

\section{Results and Discussion}
\label{sec:experiments}

We evaluate Multiphase-Diff for generating high-contrast, sharp-interface
multiphase fields through three complementary studies. First, a baseline
comparison evaluates its physical and distributional fidelity against seven
representative generative methods on three multiphase benchmarks. Second, a
component ablation study examines the roles of the bijective representation,
conservative flux residual, and local preconditioner. Third, a robustness
study tests its sensitivity to phase contrast and composition over
$\gamma=10^{1}$--$10^{5}$ and high-phase volume fractions
$v_f=0.1$--$0.9$, respectively. Together, these experiments assess the
comparative performance, mechanism, and robustness of Multiphase-Diff in the
tested high-contrast, sharp-interface regime.

\subsection{Experimental Setup}
\label{sec:experimental_setup}

\paragraph{Datasets.}
We select three complementary benchmarks that expose distinct failure modes
in high-contrast, sharp-interface multiphase fields. Case~1 considers
multi-facies Darcy flow with irregular coefficient discontinuities and a
permeability contrast of approximately $10^{3}$. Case~2 considers
gas--liquid duct flow with sharp interfaces, viscosity contrasts from $55$
to $10^{4}$, and strongly heterogeneous velocity scales. Case~3 considers
three-phase electrode conduction at a contrast of $10^{6}$, including a
near-insulating pore phase and conductive structures only one to two pixels
wide. The three cases complement one another by progressing from
coefficient discontinuity, to coupled coefficient--solution scale
heterogeneity, and finally to extreme contrast, trimodality, and
near-degenerate thin phases. They also cover Neumann, Dirichlet, and mixed
boundary conditions. Each dataset contains $10{,}000$ training and $1{,}000$
validation coefficient--solution pairs on a $64\times64$ cell-centered
grid. The governing equations, boundary conditions, and data-generation
procedures are provided in the Supplementary Material.

\paragraph{Metrics.}
We use four complementary metrics to assess the distinct requirements of
high-contrast multiphase generation. Physical Residual Fidelity
(\textbf{PRF}) measures local conservation using the
Jacobi-preconditioned finite-volume residual. The negative-coefficient rate
(\textbf{Neg}) measures whether generated coefficients remain in the
physically admissible positive domain. The worst per-phase
Wasserstein-1 distance of $\ln a$ (\textbf{$W_1$}) measures whether every
material phase is generated at the correct scale, rather than allowing an
accurately generated dominant phase to conceal failure on a minor phase.
Interface sharpness (\textbf{Sharp}) compares neighboring-cell jumps in
$\ln a$ and detects blurred or erased material boundaries. Together, they evaluate physical
consistency, feasibility, phase-wise distributional fidelity, and interface
preservation. Mathematical definitions and reference-data floors are given in the
Supplementary Material.

\paragraph{Implementation.}
All diffusion-based trained models use the same $12.78$M-parameter 2D
U-Net, except for the additional conditioning input channels required by
PG-Diffusion. We use $T=100$ diffusion steps with a cosine schedule,
$x_0$-parameterization with Min-SNR-5 weighting, a batch size of $32$, and
Adam with learning rate $10^{-4}$. Each model is trained for $100{,}000$
steps with an exponential moving average of $0.999$, and each reported
result is evaluated on $256$ generated samples. The preconditioned flux and
pointwise residual weights are set to $0.1$ and $10^{-3}$, respectively.
All experiments are implemented in PyTorch and run on a single NVIDIA
GeForce RTX~4090 GPU. Additional architecture, baseline-specific, and
sampling details are provided in the Supplementary Material.

\subsection{Baseline Comparison}
\label{sec:baseline_comparison}

We compare Multiphase-Diff with seven representative baselines spanning
data-driven generation and three major strategies for incorporating physics
into generative models. \textbf{DDPM} provides the physics-free reference.
\textbf{PG-Diffusion} supplies the residual gradient as a conditioning
input. \textbf{CoCoGen} corrects clean samples by residual descent during
inference, whereas \textbf{DiffusionPDE} guides noisy samples by
backpropagating the physical residual through the denoiser.
\textbf{FunDiff} first learns a physics-informed function autoencoder and
then generates samples using a latent rectified flow. \textbf{PIDM}
incorporates a conventional pointwise residual directly into diffusion
training, while \textbf{PIDM-log} combines the same residual with a
positive logarithmic representation. Multiphase-Diff instead places a
positivity-preserving, interface-compatible, and locally balanced physical
constraint directly in the generative objective.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{lrrrrrrrrr}
\toprule
 & DDPM & PG & CoCo & DiffPDE & FunDiff & PIDM & PIDM-log & M-Diff & Floor \\
\midrule
\multicolumn{10}{l}{(a) PRF median $\downarrow$}\\
Case 1 & $1.09\!\times\!10^{-2}$ & $1.34\!\times\!10^{-2}$ & $1.96\!\times\!10^{-2}$ & $9.76\!\times\!10^{-3}$ & $6.28\!\times\!10^{-3}$ & $9.81\!\times\!10^{-4}$ & $8.26\!\times\!10^{-4}$ & \textbf{$3.58\!\times\!10^{-4}$} & $4.60\!\times\!10^{-7}$ \\
Case 2 & $8.57\!\times\!10^{-2}$ & $1.14\!\times\!10^{-1}$ & $1.60\!\times\!10^{-1}$ & $9.18\!\times\!10^{-2}$ & $1.47\!\times\!10^{-3}$ & $4.57\!\times\!10^{-1}$ & $1.61\!\times\!10^{-3}$ & \textbf{$2.30\!\times\!10^{-4}$} & $3.70\!\times\!10^{-7}$ \\
Case 3 & $3.43\!\times\!10^{-3}$ & $3.16\!\times\!10^{-3}$ & $1.24\!\times\!10^{-3}$ & $3.23\!\times\!10^{-3}$ & $4.48\!\times\!10^{-3}$ & $1.68\!\times\!10^{-3}$ & $3.15\!\times\!10^{-3}$ & \textbf{$4.17\!\times\!10^{-4}$} & $2.30\!\times\!10^{-7}$ \\
\midrule
\multicolumn{10}{l}{(b) Negative-coefficient rate (\%) $\downarrow$}\\
Case 1 & 1.9 & 4.5 & 6.9 & 2.8 & \textbf{0.0} & 2.4 & \textbf{0.0} & \textbf{0.0} & -- \\
Case 2 & 7.0 & 11.1 & 14.8 & 8.8 & \textbf{0.0} & 43.0 & \textbf{0.0} & \textbf{0.0} & -- \\
Case 3 & 20.0 & 28.1 & 33.1 & 27.0 & \textbf{0.0} & 3.2 & \textbf{0.0} & \textbf{0.0} & -- \\
\midrule
\multicolumn{10}{l}{(c) Worst per-phase $W_1$ $\downarrow$}\\
Case 1 & 0.144 & 0.298 & 0.116 & 0.174 & 0.038 & 1.305 & 0.179 & \textbf{0.008} & -- \\
Case 2 & 1.141 & 1.140 & 1.149 & 1.187 & 1.339 & 3.397 & 1.422 & \textbf{0.933} & -- \\
Case 3 & 2.522 & 2.520 & 2.715 & 2.502 & 0.739 & 2.486 & 1.282 & \textbf{0.025} & -- \\
\midrule
\multicolumn{10}{l}{(d) Interface sharpness $W_1$ $\downarrow$}\\
Case 1 & 0.135 & 0.237 & 0.104 & 0.150 & 0.126 & 0.123 & 0.055 & \textbf{0.023} & -- \\
Case 2 & 0.120 & 0.118 & 0.099 & 0.131 & 0.045 & 0.240 & 0.128 & \textbf{0.023} & -- \\
Case 3 & 0.733 & 0.792 & 0.639 & 0.720 & 0.374 & 1.154 & 0.193 & \textbf{0.039} & -- \\
\bottomrule
\end{tabular}
\caption{Baseline comparison over 256 generated samples. M-Diff denotes Multiphase-Diff. Lower is better for all metrics; best values are bold. PRF floors are computed from held-out reference data.}
\label{tab:baseline_comparison}
\end{table*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]
    {Figures/fig1_tradeoff.pdf}
    \caption{Joint physical and distributional fidelity across the three
    complementary benchmarks. Each point denotes one generative method;
    lower PRF and lower worst-phase $W_1$ are better. Multiphase-Diff
    occupies the lower-left region in all three cases, indicating that its
    lower physical residual is not obtained by sacrificing phase-wise
    distributional fidelity.}
    \label{fig:tradeoff}
\end{figure*}

\paragraph{Case 1: Irregular Coefficient Discontinuities.}
Case~1 isolates the difficulty posed by a discontinuous coefficient field
with irregular interfaces and a low-permeability phase. Multiphase-Diff
achieves the lowest PRF, $3.58\times10^{-4}$, which is $2.3$ times lower
than the strongest baseline, while maintaining a zero negative-coefficient
rate. Its worst per-phase $W_1$ is $0.008$, close to the split-half
reference value of $0.004$, and its interface-sharpness error of $0.023$ is
also the lowest among all methods. Case~1 therefore establishes that
Multiphase-Diff can recover both the scale of a low-valued material phase
and its irregular sharp boundaries when the dominant difficulty is
concentrated in the discontinuous coefficient field.

\paragraph{Case 2: Coupled Coefficient--Solution Scale Heterogeneity.}
Case~2 is a gas--liquid system in which sharp
viscosity interfaces coexist with strongly heterogeneous velocity scales.
Multiphase-Diff obtains the lowest PRF, $2.30\times10^{-4}$, approximately
$6.4$ times lower than the next-best method and more than two orders of
magnitude below DDPM. It also maintains a zero negative-viscosity rate and
achieves the lowest interface-sharpness error, $0.023$. Its worst
per-phase $W_1$ of $0.933$ is the best among the compared methods, although
it remains above the reference value of $0.147$. This remaining discrepancy
is consistent with the sample-level imbalance among the three liquid types,
whose generated proportions differ from their nearly uniform proportions in
the training data. Case~2 shows that Multiphase-Diff remains
effective when coefficient discontinuities are coupled with strong
solution-scale heterogeneity, while also revealing that improved local
physics does not by itself guarantee an exact global mixture distribution.

\paragraph{Case 3: Extreme Contrast with Thin and Near-Degenerate Phases.}
Case~3 combines the most severe tested conditions: a conductivity contrast
of $10^{6}$, three material phases, a near-insulating pore phase, and a
conductive CBD phase only one to two pixels wide. Multiphase-Diff achieves
the lowest PRF, $4.17\times10^{-4}$, approximately three times lower than
the next-best method, with no negative conductivities. Its worst per-phase
$W_1$ is only $0.025$, compared with at least $0.739$ for every baseline,
and its interface-sharpness error of $0.039$ is approximately five times
lower than the next-best value. Some baselines match the isolated,
high-conductivity CBD mode more closely, because this is the easiest phase
to represent, but simultaneously incur large errors on the near-zero pore
phase or generate non-positive conductivities. Multiphase-Diff instead
maintains balanced fidelity across all three phases. Case~3 therefore
extends the evidence to extreme contrast, showing that Multiphase-Diff can
simultaneously preserve near-degenerate and geometrically thin phases,
sharp interfaces, positive coefficients, and local conservation.


\subsection{Component Ablations}
\label{sec:ablations}

In ablations, we remove each of Multiphase-Diff's three components in turn: the positive bijective
representation (I), the conservative flux residual (II), and the local
Jacobi preconditioner (III). Table~\ref{tab:ablations} reports the complete
results. 

\begin{table*}[t]
\centering
\caption{Component ablations on Cases 1/2/3. ``Interfaces'' denotes the
number of valid interface faces per sample, and ``worst $W_1$'' is the
largest per-phase distribution distance. The unpreconditioned model
achieves lower PRF in Cases 1 and 2 by eliminating material interfaces,
rather than by generating more faithful samples.}
\label{tab:ablations}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc}
\toprule
Variant &
PRF median &
Interfaces &
Worst per-phase $W_1$ &
Phase-fraction error \\
\midrule
Multiphase-Diff &
$3.6{\times}10^{-4}$ / $2.3{\times}10^{-4}$ / $4.2{\times}10^{-4}$ &
$64$ / $64$ / $188$ &
$0.006$ / $1.04$ / $0.025$ &
$0.045$ / $0.073$ / $0.010$ \\

$-\mathrm{I}$: affine + flux &
\multicolumn{4}{c}{Diverged (NaN at steps $300$ / $700$ / $1100$)} \\

$-\mathrm{II}$: pointwise residual &
$7.1{\times}10^{-4}$ / $1.5{\times}10^{-3}$ / $3.2{\times}10^{-3}$ &
$62$ / $0.18$ / $164$ &
$0.171$ / $1.85$ / $1.297$ &
$0.098$ / $0.080$ / $0.013$ \\

$-\mathrm{III}$: no preconditioning &
$8.5{\times}10^{-5}$ / $4.4{\times}10^{-5}$ / $1.1{\times}10^{-3}$ &
$0$ / $0$ / $2.4$ &
$2.022$ / $2.750$ / $0.982$ &
$0.316$ / $0.098$ / $0.032$ \\
\bottomrule
\end{tabular}
\end{table*}

\paragraph{Positive bijective representation.}
Removing component I causes all three runs to diverge within $1100$
training steps. Affine decoding leaves the positive coefficient domain
during early training, destabilizing the harmonic transmissibility used by
the conservative flux residual. The bijective representation is therefore
a structural prerequisite for stable flux-based training in the present
implementation, although the experiment does not establish that the
logarithmic transform is the only possible positive parameterization.

\paragraph{Conservative flux residual.}
Replacing component II with the pointwise residual consistently degrades
both physics and material fidelity. Most notably, the number of valid
interfaces in Case~2 decreases from approximately $64$ to $0.18$, while
the worst per-phase $W_1$ in Case~3 increases from $0.025$ to $1.297$.
The conservative residual is therefore essential for retaining
discontinuous and geometrically thin phases while enforcing local
conservation.

\paragraph{Local preconditioning.}
Removing component III produces the lowest PRF in Cases~1 and 2,
$8.5\times10^{-5}$ and $4.4\times10^{-5}$, but eliminates all detected
interfaces and increases the worst per-phase $W_1$ to $2.022$ and $2.750$.
The model thus lowers the residual by collapsing the coefficient contrast,
making the generated physical problem easier rather than more accurate.
Local preconditioning prevents this physics--distribution collapse by
balancing the residual according to the local flux scale.

Taken together, the ablations identify three complementary roles within
Multiphase-Diff. The bijective representation keeps the coefficient physically
admissible and enables stable flux evaluation; the conservative residual
provides an interface-compatible physics signal; and local preconditioning
prevents the model from reducing that signal by erasing material contrast.
The components therefore operate as a coupled sequence rather than as
three independent improvements. Accordingly, the ablations show that the
corresponding failure modes reappear when each component is removed, but
they do not assign an independent numerical gain to each component.

\subsection{Robustness Study}
\label{sec:robustness}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]
    {Figures/fig3_robustness.pdf}
    \caption{Robustness of Multiphase-Diff to coefficient contrast and
    phase composition. Left: PRF across contrast levels
    $\gamma=10^{1}$--$10^{5}$ at $v_f=0.5$. Right: PRF across high-phase
    volume fractions $v_f=0.1$--$0.9$ at $\gamma=10^{3}$. The
    negative-coefficient rate is zero at every tested setting.}
    \label{fig:robustness}
\end{figure*}

The three main cases evaluate Multiphase-Diff across different physical
systems, but their contrast, phase composition, geometry, and boundary
conditions vary simultaneously. To isolate sensitivity to individual
problem parameters, we construct two controlled five-point sweeps based on
Case~1. Both retain the same Darcy equation, source term, boundary
conditions, $64\times64$ grid, finite-volume solver, and training protocol.
The contrast sweep fixes the high-permeability volume fraction at
$v_f=0.5$ and varies
$\gamma\in\{10^{1},10^{2},10^{3},10^{4},10^{5}\}$. The composition sweep
fixes $\gamma=10^{3}$ and varies
$v_f\in\{0.1,0.3,0.5,0.7,0.9\}$, covering settings in which either phase
becomes a minority. Multiphase-Diff is trained independently at each
setting and evaluated using the same four metrics as in the main
comparison.

Across the contrast sweep, PRF remains within the narrow range
$3.10\times10^{-4}$--$4.07\times10^{-4}$ and the negative-coefficient rate
remains zero. The worst per-phase $W_1$ stays below $0.034$, while the
interface-sharpness error increases moderately from $0.006$ at
$\gamma=10^{1}$ to $0.021$ at $\gamma=10^{5}$. Thus, increasing the
coefficient contrast by four orders of magnitude produces only a modest
change in distributional and interface errors and no systematic
deterioration in physical consistency or feasibility.

Across the composition sweep, PRF remains in the same order of magnitude,
ranging from $2.22\times10^{-4}$ to $8.09\times10^{-4}$, with the largest
value occurring at $v_f=0.7$ rather than at either composition extreme.
The negative-coefficient rate remains zero, the worst per-phase $W_1$ is
at most $0.018$, and the interface-sharpness error remains below $0.010$.
Multiphase-Diff therefore retains both phases even when either occupies
only approximately $10\%$ of the domain. Together, the controlled sweeps
show that its performance is not tied to a particular contrast or balanced
phase composition within the tested Darcy family, complementing the
cross-physics evidence from the three main cases.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/figures/fig4_contrast_scaling.pdf}
    \caption{Conservative residual versus coefficient contrast $\gamma$. Multiphase-Diff's margin over the strongest baseline widens as $\gamma$ increases.}  % placeholder — edit
    \label{fig:contrast}
\end{figure}
\bibliographystyle{aaai2026}
\bibliography{reference}

